Kiss3DGen: Repurposing Image Diffusion Models for 3D Asset Generation

Diffusion models have achieved great success in generating 2D images. However, the quality and generalizability of 3D content generation remain limited. State-of-the-art methods often require large-scale 3D assets for training, which are challenging to collect. In this work, we introduce Kiss3DGen (Keep It Simple and Straightforward in 3D Generation), an efficient framework for generating, editing, and enhancing 3D objects by repurposing a well-trained 2D image diffusion model for 3D generation. Specifically, we fine-tune a diffusion model to generate ''3D Bundle Image'', a tiled representation composed of multi-view images and their corresponding normal maps. The normal maps are then used to reconstruct a 3D mesh, and the multi-view images provide texture mapping, resulting in a complete 3D model. This simple method effectively transforms the 3D generation problem into a 2D image generation task, maximizing the utilization of knowledge in pretrained diffusion models. Furthermore, we demonstrate that our Kiss3DGen model is compatible with various diffusion model techniques, enabling advanced features such as 3D editing, mesh and texture enhancement, etc. Through extensive experiments, we demonstrate the effectiveness of our approach, showcasing its ability to produce high-quality 3D models efficiently.

==> sec/Legacy/1_intro.tex <==
% % 背景
% The development of 3D generation is thriving these days, and various frameworks have been proposed to generate 3D assets based on multi-modal conditions such as text or images. 
% % 快速总结3D生成和2D生成模型的相关性
% As pioneer works~\cite{poole2022dreamfusion,lin2023magic3d,chen2023fantasia3d,wang2024prolificdreamer,2023luciddreamer} achieve high-quality text-to-3D generation by lifting 2D generation prior~\cite{song2020score} to 3D with optimization-based frameworks, more recent works~\cite{liu2023one2345,liu2023one2345++,liu2023zero1to3,shi2023zero123plus} extend 2D diffusion models for view-consistent object-centric image generation, then reconstruct the 3D assets by sparse-view reconstruction~\cite{}.
% Meanwhile, the emergence of large-scale 3D generative models~\cite{hong2024lrmlargereconstructionmodel,zhang2024clay,li2024craftsman} enables direct generation of 3D geometry. 

% % 展开对数据的讨论
% However, the performance of the 3D native models shows marginal superiority over the 2D-lifting methods in real-world applications, as we exhibited in Sec.~\ref{sec:evaluation}. %需要可视化支撑
% % 引出我们的方法
% Meanwhile, we surprisingly find that pretrained 2D diffusion transformer models (DITs)~\cite{} can easily harness sophisticated 3D asset generation after simple finetuning on a few 3D data.
% Specifically, we 

